Violet: Architecturally Exposed Orchestration, Movement, and Placement for Generalized Deep Learning

Deep learning and hardware for it has garnered immense academic and industry interest in the past 5 years, with many novel proposals. However, the state-of-art remains NVIDIA's TensorCore-based systems that provide top-of-line performance and coverage across a wide-spectrum of deep learning applications. In this paper, we first identify four key problems any new DL solution must solve: 1) Data orchestration, 2) Data movement, 3) Work placement and blending these to achieve 4) Coverage across different types of DL applications. With this as a guide, we propose Violet, a novel architecture with roots in multicore SIMD which balances the responsibilities for these four problems between the architecture, microarchitecture and software stack. Compared to the NVIDIA A100 GPU, we find Violet achieves geo-mean 2.4X/10.6X and 2.1X/9.5X performance/efficiency for inference and training across the MLPerf benchmark suite. We present detailed operator-level analysis of the MLPerf benchmark suite, extracting out key behaviors - with implications for architecture research beyond this paper, that underpin the speedup and efficiency. Overall, this paper motivates the importance of balance, that the break down of responsibilities must be thought through carefully in order to compete with incumbent architecture designs.

==> figs/shape-table-old.tex <==

\begin{tabular}{llrrrl}
\hline
\multicolumn{1}{c}{\textbf{Op}} & +TP & -TP & \multicolumn{1}{c}{\textbf{A100}} & \multicolumn{1}{c}{\textbf{Comments}} \\ \hline
\multicolumn{5}{c}{\textbf{Resnet50 (All 2D Conv.)}} \\ \hline
I 14$^2$ 256-\textgreater{}256 f=3 s1 & 82\% & 68\% & 14\% & \tag{SS} \tag{LC} \\ % ex
I 56$^2$ 64-\textgreater{}64 f=3 s1 & 90\% & 78\% & 12\% & \tag{LS} \tag{SC} \\ % ex
I 28$^2$ 128-\textgreater{}128 f=3 s1 & 80\% & 82\% & 16\% & \tag{SS} \\ % ex
I 14$^2$ 256-\textgreater{}1024 f=1 s1 & 69\% & 93\% & 8\% & \tag{F1} \tag{LC} \tag{A-} \\ % ex
I 14$^2$ 1024-\textgreater{}256 f=1 s1 & 66\% & 72\% & 9\% & \tag{SS} \tag{BP} \\ % ex
T 14$^2$ 256-\textgreater{}256 f=3 s1 & 25\% & 5\% & 15\% & \tag{DW} \tag{SS} \\ % comm
T 56$^2$ 64-\textgreater{}64 f=3 s1 & 61\% & 6\% & 11\% & \tag{DW} \tag{LS} \tag{SC} \\ % comm
T 28$^2$ 128-\textgreater{}128 f=3 s1 & 65\% & 6\% & 14\% & \tag{DW} \tag{LS} \tag{SC} \\ % comm
T 14$^2$ 256-\textgreater{}1024 f=1 s1 & 34\% & 15\% & 8\% & \tag{DW} \tag{F1} \tag{LC} \\ % comm
T 14$^2$ 1024-\textgreater{}256 f=1 s1 & 67\% & 16\% & 9\% & \tag{DW} \tag{F1} \tag{LC} \\ % comm
\hline
\multicolumn{5}{c}{\textbf{SSD-Resnet34 (All 2D Conv.)}} \\ \hline
I 150$^2$ 256-\textgreater{}256 f=3 s1 & 94\% & 46\% & 53\% & \tag{LS} \tag{LC} \tag{GP} \\ % ex
I 150$^2$ 128-\textgreater{}128 f=3 s1 & 97\% & 82\% & 37\% & \tag{LS} \tag{LC} \\ % ex
I 300$^2$ 64-\textgreater{}64 f=3 s1 & 99\% & 74\% & 26\% & \tag{LS} \\ % ex
I 150$^2$ 128-\textgreater{}256 f=3 s1 & 98\% & 67\% & 43\% & \tag{LS} \tag{LC} \\ % ex
I 150$^2$ 256-\textgreater{}512 f=3 s2 & 77\% & 17\% & 45\% & \tag{S2} \\ % ex
T 38$^2$ 256-\textgreater{}256 f=3 s1 & 53\% & 5\% & 37\% & \tag{DW} \tag{SS} \tag{LC} \\ % comm
T 38$^2$ 128-\textgreater{}128 f=3 s1 & 62\% & 6\% & 20\% & \tag{DW} \tag{SS} \tag{LC} \\ % comm
T 75$^2$ 64-\textgreater{}64 f=3 s1 & 69\% & 6\% & 14\% & \tag{DW} \tag{SS} \tag{LC} \\ % comm
T 38$^2$ 128-\textgreater{}256 f=3 s1 & 45\% & 6\% & 27\% & \tag{DW} \tag{SS} \tag{LC} \\ % comm
T 38$^2$ 256-\textgreater{}512 f=3 s2 & 25\% & 3\% & 27\% & \tag{DW} \tag{SS} \tag{LC} \\ % comm
\hline
\multicolumn{5}{c}{\textbf{UNet (All 3D Conv.)}} \\ \hline
I 32$^3$ 32-\textgreater{}32 f=3 s1 & 24\% & 49\% & 22\% & \tag{BP} \tag{LS} \tag{SC} \\ % ex
I 32$^3$ 64-\textgreater{}32 f=3 s1 & 24\% & 99\% & 15\% & \tag{BP} \tag{LS} \tag{SC} \\ % ex
I 32$^3$ 64-\textgreater{}64 f=3 s1 & 49\% & 99\% & 28\% & \tag{BP} \tag{LS} \tag{SC} \\ % ex
I 32$^3$ 128-\textgreater{}64 f=3 s1 & 49\% & 99\% & 35\% & \tag{BP} \tag{LS} \tag{LC} \\ % ex
I 32$^3$ 128-\textgreater{}128 f=3 s1 & 99\% & 99\% & 53\% & \tag{BP} \tag{LS} \tag{LC} \\ % ex
T 32$^3$ 32-\textgreater{}32 f=3 s1 & 27\% & 8\% & 16\% & \tag{DW} \tag{LS} \tag{SC} \\ % ex
T 32$^3$ 64-\textgreater{}32 f=3 s1 & 39\% & 8\% & 19\% & \tag{DW} \tag{LS} \tag{SC} \\ % ex
T 32$^3$ 64-\textgreater{}64 f=3 s1 & 57\% & 8\% & 35\% & \tag{DW} \tag{LS} \tag{SC} \\ % ex
T 32$^3$ 128-\textgreater{}64 f=3 s1 & 71\% & 8\% & 43\% & \tag{DW} \tag{LS} \tag{LC} \\ % ex
T 32$^3$ 128-\textgreater{}128 f=3 s1 & 94\% & 8\% & 57\% & \tag{DW} \tag{LS} \tag{LC} \\ % ex
\hline
\multicolumn{5}{c}{\textbf{BERT-Large}} \\ \hline
I Fc(2848x1024x1024) & 87\% & 76\% & 32\% & \tag{LM} \tag{LN} \tag{LK} \\ % ex
I Fc(2848x4096x1024) & 91\% & 31\% & 93\% & \tag{LM} \tag{LN} \tag{LK} \\ % ex
I Fc(2848x1024x4096) & 90\% & 52\% & 31\% & \tag{LM} \tag{LN} \tag{LK} \\ % ex
I Mm(178x178x64) & 27\% & 27\% & 8\% & \tag{LL} \tag{SM} \tag{SN} \\ % ex
I Mm(178x64x178) & 14\% & 14\% & 6\% & \tag{LL} \tag{SM} \tag{SN} \\ % ex
T Fc(4064x1024x1024) & 83\% & 14\% & 95\% & \tag{TP} \tag{LM} \tag{LN} \tag{LK} \\ % comm
T Fc(4064x4096x1024) & 83\% & 14\% & 47\% & \tag{TP} \tag{LM} \tag{LN} \tag{LK} \\ % comm
T Fc(4064x1024x4096) & 83\% & 14\% & 93\% & \tag{TP} \tag{LM} \tag{LN} \tag{LK} \\ % comm
T Mm(254x254x64) & 2\% & 2\% & 9\% & \tag{TP} \tag{LL} \tag{SM} \tag{SN} \\ % comm
T Mm(254x64x254) & 5\% & 5\% & 17\% & \tag{TP} \tag{LL} \tag{SM} \tag{SN} \\ % comm
\hline
\multicolumn{5}{c}{\textbf{RNN-T}} \\ \hline
I Lstm(512x4096x2048) & 65\% & 18\% & 22\% & \tag{EW} \tag{LN} \tag{LK} \\ % mem
I Lstm(512x4096x3072) & 50\% & 36\% & 24\% & \tag{EW} \tag{LN} \tag{LK} \\ % mem
I Lstm(512x4096x1264) & 91\% & 56\% & 16\% & \tag{EW} \tag{LN} \tag{LK} \\ % mem
I Lstm(512x1280x640) & 48\% & 65\% & 6\% & \tag{EW} \tag{SK} \\ % mem
I Fc(512x1344x512) & 46\% & 71\% & 11\% & \tag{EW} \tag{BP} \\ % mem
T Lstm(512x4096x2048) & 41\% & 11\% & 19\% & \tag{TP} \tag{EW} \tag{LN} \tag{LK} \\ % comm
T Lstm(512x4096x3072) & 41\% & 11\% & 23\% & \tag{TP} \tag{EW} \tag{LN} \tag{LK} \\ % comm
T Lstm(512x4096x1264) & 36\% & 11\% & 16\% & \tag{TP} \tag{EW} \tag{LN} \tag{LK} \\ % comm
T Lstm(512x1280x640) & 47\% & 14\% & 5\% & \tag{TP} \tag{EW} \tag{SK} \\ % comm
T Fc(512x1344x512) & 42\% & 14\% & 7\% & \tag{TP} \tag{EW} \\ % comm
\hline
\end{tabular}


==> figs/util-table.tex <==

\begin{tabular}{lrrrr}
 & \multicolumn{2}{c}{A100}                              & \multicolumn{2}{c}{\ourarch}                           \\
 & \multicolumn{1}{c}{Small} & \multicolumn{1}{c}{Large} & \multicolumn{1}{c}{Small} & \multicolumn{1}{c}{Large} \\ \hline

Resnet50 (I)  & 2.68 \% & 48.29 \% & 10.74 \% & 59.99 \% \\
SSD-Resnet34 (I)  & 35.97 \% & 62.63 \% & 77.26 \% & 90.15 \% \\
UNet (I)  & 28.14 \% & 28.23 \% & 34.21 \% & 34.71 \% \\
BERT-Large (I)  & 12.08 \% & 56.85 \% & 20.55 \% & 81.15 \% \\
13594.4 Float16 14034042880 312000000000000.0
RNN-T (I)  & 0.32 \% & 61.15 \% & 0.14 \% & 63.68 \% \\
\hline
Resnet50 (T)  & 1.52 \% & 25.86 \% & 4.88 \% & 25.81 \% \\
SSD-Resnet34 (T)  & 2.22 \% & 40.82 \% & 6.06 \% & 41.98 \% \\
UNet (T)  & 27.98 \% & 31.93 \% & 6.78 \% & 32.46 \% \\
BERT-Large (T)  & 0.31 \% & 42.11 \% & 19.87 \% & 41.11 \% \\
RNN-T (T)  & 0.51 \% & 13.00 \% & 0.10 \% & 40.56 \% \\
\hline

\end{tabular}



==> relwork.tex <==
EyerissV2 and Simba evaluate only inference for convolution and/or linear layers, and are explicitly designed as inference-only accelerators. Sigma only provides mappings for DNN workloads, with no support for convolution inference or training. MAGNet deliberately eschew coverage in order to produce a single accelerator configuration -- with a fixed set of solutions to these problems -- optimized for one workload. This limited design space does not lend to designs which could achieve coverage with better solutions to data orchestration, data movement and work placement.

Sigma employs its FlexDPE, using a software programmed, fan-out and fan-in network for data orchestration which we find is over-engineered for DL workloads (We discuss this more in Sec~\ref{sec:arch-orch}). Software is responsible for optimizing orchestration by extracting out what configurations will most benefit the computation given -- a complex task.

Existing solutions such as EyerissV2 employ entirely software-scheduled data movement through its circuit-switched HM-NoC, meaning software must determine routes for every input element and embed this within the static configuration for every switch. If routing needs exceed available resources, a particular dataflow cannot map to this NoC. Simba, in contrast, uses a dynamic NoC with three levels of hierarchy and its Global PE and Controller can multicast data to local or remote PEs.

For Simba, work placement must account for relatively expensive cross-chiplet communication, and must understand the constraints imposed by the specific inter- and intra-chiplet topology. Eyeriss must understand the routing resource topology in order to place work in a way that can be routed by its HM-NoC.
%%%%%%


Simba and MAGNet both employ conventional style SIMD for data orchestration but lack the flexibility for differing layouts and shapes afforded by \ourarch{}'s Transpose Engine. Sigma is interesting in that it has highly configurable data orchestration, but this configurability comes at the cost of additional routing in for the Benes fan-out and tree fan-in network, where \ourarch{}'s transpose engine afford high efficiency across MLPerf with a relatively simple design (just registers). EyerissV2's achieves data orchestration by only including two single-element MAC units per PE, making them much finer-grained compute resources compared to \ourarch{}. This means scaling EyerissV2's PE design to the same peak compute as \ourarch{} would require an order of magnitude larger NoC, complicating data movement.


Simba includes multi-cast functionality in its Globla PE and controller core, affording a  software-managed multi-cast. However, Simba's Global PE is the only element on the chiplet that is able to do near-memory compute where \ourarch{} allows all compute resources to participate in this type of operation. EyerissV2 requires entirely statically scheduled data movement, where every route through their NoC is planned by software ahead of execution, making it effectively impossible to support data-dependent control flow at the intra-operator level. Sigma and MAGNet both use a conventional mesh NoC, with individual cores issuing read requests -- not ``push'' style data movement that \ourarch{} uses.


Work placement for EyerissV2 involves co-planning static data movement with assigning work to PEs. This process is solved for convolution by employing row-stationary dataflow, there is substantial lift in supporting new operations. Sigma and MAGNet both can rely on dynamic data movement to make work placement easier, but will incur lots of request traffic and data movement for element-wise operations that are not arithmetically intense. Simba also has the benefit of dynamic data movement, but its chiplet based design adds an architectural level of hierarchy that must be considered by the placement scheme, complicating placement.

